PDM-SSD: Single-Stage Three-Dimensional Object Detector With Point Dilation

Current Point-based detectors can only learn from the provided points, with limited receptive fields and insufficient global learning capabilities for such targets. In this paper, we present a novel Point Dilation Mechanism for single-stage 3D detection (PDM-SSD) that takes advantage of these two representations. Specifically, we first use a PointNet-style 3D backbone for efficient feature encoding. Then, a neck with Point Dilation Mechanism (PDM) is used to expand the feature space, which involves two key steps: point dilation and feature filling. The former expands points to a certain size grid centered around the sampled points in Euclidean space. The latter fills the unoccupied grid with feature for backpropagation using spherical harmonic coefficients and Gaussian density function in terms of direction and scale. Next, we associate multiple dilation centers and fuse coefficients to obtain sparse grid features through height compression. Finally, we design a hybrid detection head for joint learning, where on one hand, the scene heatmap is predicted to complement the voting point set for improved detection accuracy, and on the other hand, the target probability of detected boxes are calibrated through feature fusion. On the challenging Karlsruhe Institute of Technology and Toyota Technological Institute (KITTI) dataset, PDM-SSD achieves state-of-the-art results for multi-class detection among single-modal methods with an inference speed of 68 frames. We also demonstrate the advantages of PDM-SSD in detecting sparse and incomplete objects through numerous object-level instances. Additionally, PDM can serve as an auxiliary network to establish a connection between sampling points and object centers, thereby improving the accuracy of the model without sacrificing inference speed. Our code will be available at https://github.com/AlanLiangC/PDM-SSD.git.

==> 05_conclusion.tex <==
% \qy{In this paper, we propose an efficient single-stage framework called \nickname{} for 3D object detection. Considering the task of object detection inherently focuses on the foreground points, we propose an instance-aware learning-based downsampling way to automatically select the sparse yet important instance points. In addition, a dedicated contextual centroid perception module is proposed to fully exploit the geometrical structure around the bounding boxes. Extensive experiments conducted on the KITTI detection benchmark demonstrated the superior efficiency and accuracy of the proposed \nickname{}. \revise{In future work, we will further tackle extreme cases such as overlapped bounding boxes.}}

%This paper presents a new point-based single-stage 3D object detection networks, named \nickname{}. With novel instance-aware downsampling strategy and centroid rally module, we can effectively and efficiently achieve muti-class 3D object detection in a bottom-up manner.  Our \nickname{} achieves the best results among pure point-based methods, and provides a state-of-the-art efficiency than existing LiDAR detectors. In the future, we will focus on designing an efficient network to achieve real-time and robust 3D detection in 360-degree LiDAR scenes.

\qy{In this paper, we propose an efficient solution termed \nickname{} for point-based 3D object detection in LiDAR point clouds. Considering the task of object detection inherently focuses on the foreground information, we propose an instance-aware learning-based downsampling way to automatically select the sparse yet important instance points. Additionally, a dedicated contextual centroid perception module is proposed to fully exploit the geometrical structure around the bounding boxes. Extensive experiments conducted on three detection benchmarks demonstrated the superior efficiency and accuracy of the proposed \nickname{}. 
}

\smallskip\noindent\textbf{Limitations.} Although the proposed \nickname{} can achieve remarkable efficiency in object detection of large-scale LiDAR points clouds, it also has limitations. \textit{e.g.,} the instance-aware sampling relies on the semantic prediction of each point, which is susceptible to class imbalances distribution. For future work, we will further explore advanced techniques to alleviate the imbalanced issue.



==> SPSNet_IA_kitti.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{hhline}


\begin{table}[t]
\centering
\arrayrulecolor{black}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c||ccc|ccc|ccc|ccc} 
\arrayrulecolor{black}\hline
\multirow{3}{*}{Method}                                                                           & \multirow{3}{*}{Structure}                                        & \multicolumn{6}{c}{AP\_\{3D\}@Cyclist(IoU=0.5)}                                                                                                                                                                 & \multicolumn{6}{c}{BEV(IoU=0.5)}                                                                                                                                                                                 \\ 
\arrayrulecolor{black}\cline{3-14}
                                                                                                  &                                                                   & \multicolumn{3}{c}{R11}                                                                                & \multicolumn{3}{c}{R40}                                                                                & \multicolumn{3}{c}{R11}                                                                                & \multicolumn{3}{c}{R40}                                                                                 \\
                                                                                                  &                                                                   & Easy                             & Moderate                         & Hard                             & Easy                             & Moderate                         & Hard                             & Easy                             & Moderate                         & Hard                             & Easy                             & Moderate                         & Hard                              \\ 
\arrayrulecolor{black}\cline{1-2}\arrayrulecolor{black}\cline{3-4}\arrayrulecolor{black}\cline{5-5}\arrayrulecolor{black}\cline{6-7}\arrayrulecolor{black}\cline{8-8}\arrayrulecolor{black}\cline{9-10}\arrayrulecolor{black}\cline{11-11}\arrayrulecolor{black}\cline{12-14}
VoxelNet                                                                                          & Voxel-based                                                       & 67.17                            & 47.65                            & 45.11                            & -                                & -                                & -                                & 74.41                            & 52.18                            & 52.49                            & -                                & -                                & -                                 \\
PointPillars                                                                                      & Voxel-based                                                       & 86.47                            & 68.94                            & 66.72                            & 89.81                            & 69.71                            & 66.91                            & 86.66                            & 67.21                            & 66.72                            & 90.01                            & 67.45                            & 66.91                             \\
SECOND                                                                                            & Voxel-based                                                       & 80.61                            & 67.14                            & 63.11                            & 82.97                            & 66.74                            & 62.78                            & 84.02                            & 70.7                             & 65.48                            & 88.04                            & 71.16                            & 66.89                             \\
SECOND-iou                                                                                        & Voxel-based                                                       & 80.44                            & 64.26                            & 60.19                            & 83.16                            & 63.75                            & 60.24                            & 84.64                            & 66.83                            & 63.43                            & 86.45                            & 67.73                            & 63.38                             \\
TANet                                                                                             & Voxel-based                                                       & 85.98                            & 64.95                            & 60.4                             & -                                & -                                & -                                & -                                & -                                & -                                & -                                & -                                & -                                 \\
Part-A2                                                                                           & Voxel-based                                                       & 85.5                             & 69.93                            & 65.48                            & 90.4                             & 70.1                             & 66.9                             & 86.88                            & 73.32                            & 70.84                            & 91.93                            & 74.6                             & 70.61                             \\
Part-A2-free                                                                                      & Voxel-based                                                       & \textbf{\textcolor{blue}{87.95}} & \textcolor{red}{\textbf{74.29}}  & \textbf{\textcolor{blue}{69.91}} & 91.92                            & \textbf{\textcolor{blue}{75.33}} & \textbf{\textcolor{blue}{70.59}} & \textbf{\textcolor{blue}{88.75}} & \textcolor{red}{\textbf{76.31}}  & \textcolor{red}{\textbf{73.68}}  & 93.23                            & \textcolor{red}{\textbf{78.51}}  & \textcolor{red}{\textbf{73.94}}   \\
SASSD                                                                                             & Voxel-based                                                       & 82.8                             & 63.37                            & 61.6                             & -                                & -                                & -                                & 86.78                            & 71.54                            & 65.85                            & -                                & -                                & -                                 \\ 
\arrayrulecolor{black}\cline{1-2}\arrayrulecolor{black}\cline{3-4}\arrayrulecolor{black}\cline{5-5}\arrayrulecolor{black}\cline{6-7}\arrayrulecolor{black}\cline{8-8}\arrayrulecolor{black}\cline{9-10}\arrayrulecolor{black}\cline{11-11}\arrayrulecolor{black}\cline{12-14}
PV-RCNN                                                                                           & Point-Voxel                                                       & 84.3                             & 69.29                            & 63.59                            & 87.05                            & 69.52                            & 65.19                            & 88.38                            & 73.62                            & 70.77                            & 93.36                            & 75.04                            & 70.44                             \\ 
\arrayrulecolor{black}\cline{1-2}\arrayrulecolor{black}\cline{3-4}\arrayrulecolor{black}\cline{5-5}\arrayrulecolor{black}\cline{6-7}\arrayrulecolor{black}\cline{8-8}\arrayrulecolor{black}\cline{9-10}\arrayrulecolor{black}\cline{11-11}\arrayrulecolor{black}\cline{12-14}
PointRCNN                                                                                         & Point-based                                                       & 86.76                            & 71.68                            & 65.77                            & 91.94                            & 70.98                            & 66.72                            & 88.41                            & 74.31                            & 67.96                            & 93.91                            & 74.71                            & 70.26                             \\
PointRCNN-iou                                                                                     & Point-based                                                       & 86.36                            & 70.99                            & 66.23                            & 91.48                            & 71.46                            & 66.74                            & 88.51                            & 74.54                            & 68.12                            & \textbf{\textcolor{blue}{94.06}} & 75.07                            & 70.22                             \\
IA-SSD                                                                                            & Point-based                                                       & 87.28                            & 72.28                            & 66.67                            & \textbf{\textcolor{blue}{91.98}} & 72.73                            & 68.14                            & 88.27                            & 73.72                            & 70.65                            & 93.3                             & 74.81                            & 70.68                             \\
\rowcolor[rgb]{0.816,0.808,0.808} {\cellcolor[rgb]{0.816,0.808,0.808}}                            & {\cellcolor[rgb]{0.816,0.808,0.808}}                              & \textbf{\textcolor{red}{88.16}}  & \textbf{\textcolor{blue}{74.01}} & \textbf{\textcolor{red}{71.2}}   & \textbf{\textcolor{red}{93.16}}  & \textbf{\textcolor{red}{75.51}}  & \textbf{\textcolor{red}{71.1}}   & \textbf{\textcolor{red}{93.58}}  & \textbf{\textcolor{blue}{75.03}} & \textbf{\textcolor{blue}{72.72}} & \textbf{\textcolor{red}{95.39}}  & \textbf{\textcolor{blue}{77.57}} & \textbf{\textcolor{blue}{73.22}}  \\
\rowcolor[rgb]{0.816,0.808,0.808} \multirow{-2}{*}{{\cellcolor[rgb]{0.816,0.808,0.808}}SPSNet-IA} & \multirow{-2}{*}{{\cellcolor[rgb]{0.816,0.808,0.808}}Point-based} & \textbf{0.88}                    & \textbf{1.73}                    & \textbf{4.53}                    & \textbf{1.18}                    & \textbf{2.78}                    & \textbf{2.96}                    & \textbf{5.31}                    & \textbf{1.31}                    & \textbf{2.07}                    & \textbf{2.09}                    & \textbf{2.76}                    & \textbf{2.54}                     \\
\hhline{>{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}|b|-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}---}
\end{tabular}
}
\end{table}

==> SPSNet_SIA_car.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}

\begin{table}
	\centering
	\resizebox{\textwidth}{!}{
	\begin{tabular}{c|c|c||ccc|ccc} 
		\cline{1-1}\cmidrule[\heavyrulewidth]{2-9}
		\multirow{3}{*}{Method} & \multirow{3}{*}{Structure} & \multirow{3}{*}{Type} & \multicolumn{3}{c|}{3D(IoU=0.7)} & \multicolumn{3}{c}{BEV(IoU=0.7)}  \\ 
		\cline{4-9}
		&                            &                       & \multicolumn{3}{c|}{R40}         & \multicolumn{3}{c}{R40}           \\
		&                            &                       & Easy  & Moderate & Hard          & Easy  & Moderate & Hard           \\ 
		\hline
		VoxelNet                & Voxel-based                & 1-stage               & 77.47 & 65.11    & 57.73         & 87.95 & 78.39    & 71.29          \\
		PointPillars            & Voxel-based                & 1-stage               & 82.58 & 74.31    & 68.99         & 90.07 & 86.56    & 82.81          \\
		SECOND                  & Voxel-based                & 1-stage               & 84.65 & 75.96    & 68.71         & 89.39 & 83.77    & 78.59          \\
		3DIoULoss               & Voxel-based                & 2-stage               & 86.16 & 76.5     & 71.39         & 90.23 & 86.61    & 86.37          \\
		TANet                   & Voxel-based                & 1-stage               & 84.39 & 75.94    & 68.82         & 91.58 & 86.54    & 81.19          \\
		Part-A2                 & Voxel-based                & 2-stage               & 87.81 & 78.49    & 73.51         & 91.7  & 87.79    & 84.61          \\
		CIASSD                  & Voxel-based                & 1-stage               & 89.59 & 80.28    & 72.87         & 93.74 & 89.84    & 82.39          \\
		SASSD                   & Voxel-based                & 1-stage               & 88.75 & 79.79    & 74.61         & 93.74 & 89.84    & 82.39          \\
		Associate-3Det          & Voxel-based                & 1-stage               & 85.99 & 77.4     & 70.53         & 91.4  & 88.09    & 82.96          \\
		SVGA-Net                & Voxel-based                & 1-stage               & 87.33 & 80.47    & 75.91         & -     & -        & -              \\ 
		\hline
		Fast Point R-CNN        & Point-Voxel                & 2-stage               & 85.29 & 77.4     & 70.24         & 90.87 & 87.84    & 80.52          \\
		STD                     & Point-Voxel                & 2-stage               & 87.92 & 79.71    & 75.09         & -     & -        & -              \\
		PV-RCNN                 & Point-Voxel                & 2-stage               & 90.25 & 81.43    & 76.82         & 94.98 & 90.62    & 86.14          \\
		EQ-PVRCNN               & Point-Voxel                & 2-stage               & 90.13 & 82.01    & 77.53         & 94.55 & 89.09    & 86.42          \\
		VIC-Net                 & Point-Voxel                & 1-stage               & 88.25 & 80.61    & 75.83         & -     & -        & -              \\
		HVPR                    & Point-Voxel                & 1-stage               & 86.38 & 77.92    & 73.04         & -     & -        & -              \\ 
		\hline
		PointRCNN               & Point-based                & 2-stage               & 86.96 & 75.64    & 70.7          & 92.13 & 87.39    & 82.72          \\
		3D IoU-Net              & Point-based                & 2-stage               & 87.96 & 79.03    & 72.78         & 94.76 & 88.38    & 81.93          \\
		3DSSD                   & Point-based                & 1-stage               & 88.36 & 79.57    & 74.55         & 92.66 & 89.02    & 85.86          \\
		IA-SSD                  & Point-based                & 1-stage               & 88.34 & 80.13    & 75.04         & 92.79 & 89.333   & 84.35          \\
		IA-SSD*                 & Point-based                & 1-stage               & 87.67 & 79.4     & 74.22         & -     & -        & -              \\
		DBQ-SSD                 & Point-based                & 1-stage               & 87.93 & 79.39    & 74.4          & -     & -        & -              \\
		PDM-SSD                 & Point-based                & 1-stage               & 88.74 & 80.17    & 75.13         & 92.77 & 89.52    & 85.32         
	\end{tabular}}
\end{table}

==> SPSNet_SIA_car_0.5.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{hhline}


\begin{table}
\centering
\arrayrulecolor{black}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc} 
\arrayrulecolor{black}\hline
\multirow{3}{*}{Method}                                                                            & \multicolumn{6}{c}{AP\_\{3D\}@Car(IoU=0.5)}                                                        & \multicolumn{6}{c}{AP\_\{BEV\}@Car(IoU=0.5)}                                                        \\ 
\arrayrulecolor{black}\cline{2-13}
                                                                                                   & \multicolumn{3}{c|}{R11}                         & \multicolumn{3}{c|}{R40}                        & \multicolumn{3}{c|}{R11}                        & \multicolumn{3}{c}{R40}                           \\
                                                                                                   & Easy           & Moderate       & Hard           & Easy          & Moderate       & Hard           & Easy          & Moderate       & Hard           & Easy           & Moderate       & Hard            \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-3}\arrayrulecolor{black}\cline{4-4}\arrayrulecolor{black}\cline{5-6}\arrayrulecolor{black}\cline{7-7}\arrayrulecolor{black}\cline{8-9}\arrayrulecolor{black}\cline{10-10}\arrayrulecolor{black}\cline{11-13}
IA-SSD                                                                                             & 90.74          & 90.14          & 89.65          & 96.24         & 95.44          & 94.86          & 90.74         & 90.16          & 89.72          & 96.25          & 95.53          & 95.03           \\
\rowcolor[rgb]{0.816,0.808,0.808} {\cellcolor[rgb]{0.816,0.808,0.808}}                             & 96.19          & 90.17          & 89.69          & 98.04         & 95.5           & 94.99          & 96.24         & 95.81          & 89.75          & 98.07          & 97.28          & 95.11           \\
\rowcolor[rgb]{0.816,0.808,0.808} \multirow{-2}{*}{{\cellcolor[rgb]{0.816,0.808,0.808}}SPSNet-SIA} & \textbf{+5.45} & \textbf{+0.03} & \textbf{+0.04} & \textbf{+1.8} & \textbf{+0.06} & \textbf{+0.13} & \textbf{+5.5} & \textbf{+5.65} & \textbf{+0.03} & \textbf{+1.82} & \textbf{+1.75} & \textbf{+0.08}  \\
\hhline{>{\arrayrulecolor{black}}->{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}---}
\end{tabular}
}
\end{table}

==> car_pedstrain.tex <==
% \usepackage{multirow}
% \usepackage{hhline}
% \usepackage{colortbl}


\begin{table}[t]
\centering
\arrayrulecolor{black}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc} 
\arrayrulecolor{black}\toprule
\multirow{3}{*}{Method}                     & \multicolumn{6}{c}{AP\_\{3D\}@Car(IoU=0.7)}         & \multicolumn{6}{c}{AP\_\{3D\}@Pedestrain(IoU=0.5)}                       \\ 
\arrayrulecolor{black}\cline{2-13}
                                            & \multicolumn{3}{c|}{R11} & \multicolumn{3}{c|}{R40} & \multicolumn{3}{c|}{R11} & \multicolumn{3}{c|}{R40}                      \\
                                            & Easy  & Moderate & Hard  & Easy  & Moderate & Hard  & Easy  & Moderate & Hard  & Easy  & Moderate & \multicolumn{1}{c|}{Hard}  \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-3}\arrayrulecolor{black}\cline{4-4}\arrayrulecolor{black}\cline{5-6}\arrayrulecolor{black}\cline{7-7}\arrayrulecolor{black}\cline{8-9}\arrayrulecolor{black}\cline{10-10}\arrayrulecolor{black}\cline{11-12}\arrayrulecolor{black}\cline{13-13}
IA-SSD                                      & 88.78 & 79.12    & 78.12 & 89.52 & 82.86    & 80.05 & 59.82 & 56.01    & 51.16 & 59.92 & 55.29    & 49.77                      \\
\rowcolor[rgb]{0.816,0.808,0.808} SPSNet-IA & 88.91 & 79.13    & 78.06 & 89.66 & 82.84    & 79.93 & 60.37 & 57.02    & 51.75 & 60.61 & 55.93    & 51.11                      \\
\hhline{->{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}-->{\arrayrulecolor{black}}->{\arrayrulecolor{black}}---}
\end{tabular}
}
\end{table}

==> drop.tex <==
% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table}
\centering
\arrayrulecolor{black}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c||cccccccccccc} 
\arrayrulecolor{black}\hline
\multicolumn{2}{c||}{}                 & 0      & 10     & 20     & 40     & 70     & 100    & 150    & 200    & 150    & 300    & 400    & 500     \\ 
\arrayrulecolor{black}\hline
\multirow{2}{*}{Average}   & Random    & 71.03~ & 69.56~ & 69.54~ & 69.84~ & 68.25~ & 67.06~ & 65.45~ & 62.24~ & 60.54~ & 57.38~ & 53.72~ & 52.45~  \\
                           & Stability & 71.03~ & 62.42~ & 61.56~ & 60.00~ & 57.04~ & 56.25~ & 52.45~ & 48.34~ & 44.75~ & 42.67~ & 38.92~ & 33.02~  \\ 
\cline{1-1}\arrayrulecolor{black}\cline{2-2}\arrayrulecolor{black}\cline{3-14}
\multirow{2}{*}{Car}       & Random    & 82.01~ & 81.84~ & 81.84~ & 81.61~ & 80.82~ & 79.49~ & 78.42~ & 73.53~ & 73.25~ & 72.88~ & 71.12~ & 69.13~  \\
                           & Stability & 82.01~ & 81.52~ & 81.57~ & 81.14~ & 80.04~ & 78.55~ & 76.25~ & 72.96~ & 72.71~ & 71.69~ & 68.89~ & 65.54~  \\ 
\cline{1-1}\arrayrulecolor{black}\cline{2-2}\arrayrulecolor{black}\cline{3-14}
\multirow{2}{*}{Pedstrain} & Random    & 55.66~ & 52.55~ & 52.19~ & 52.87~ & 52.56~ & 50.18~ & 47.63~ & 45.30~ & 41.11~ & 36.84~ & 33.52~ & 34.62~  \\
                           & Stability & 55.66~ & 37.35~ & 36.63~ & 35.86~ & 32.08~ & 30.30~ & 28.92~ & 22.93~ & 18.92~ & 16.51~ & 17.30~ & 9.42~   \\ 
\cline{1-1}\arrayrulecolor{black}\cline{2-2}\arrayrulecolor{black}\cline{3-14}
\multirow{2}{*}{Cyclist}   & Random    & 75.41~ & 74.30~ & 74.59~ & 75.04~ & 71.38~ & 71.53~ & 70.29~ & 67.88~ & 67.25~ & 62.43~ & 56.52~ & 53.60~  \\
                           & Stability & 75.41~ & 68.40~ & 66.48~ & 62.99~ & 58.99~ & 59.89~ & 52.18~ & 49.15~ & 42.62~ & 39.81~ & 30.58~ & 24.09~  \\
\cline{1-1}\arrayrulecolor{black}\cline{2-2}\arrayrulecolor{black}\cline{3-14}
\end{tabular}
}
\end{table}

==> parms.tex <==
% \usepackage{booktabs}


\begin{table}
	\centering
	\caption{The parameters and GFLOPs of PDM-SSD}
	\begin{tabular}{c|cccc} 
		\toprule
		& Backbone & Neck & Head  & All    \\ 
		\hline
		Parms (MB) & 0.51     & 0.53 & 2.31  & 3.3    \\
		GFLOPs     & 4.25     & 2.84 & 14.76 & 21.85  \\
		\bottomrule
	\end{tabular}
\label{tabel7}
\end{table}
